Bayesian Models of Data Streams with Hierarchical Power Priors

Making inferences from data streams is a pervasive problem in many modern data analysis applications. But it requires to address the problem of continuous model updating and adapt to changes or drifts in the underlying data generating distribution. In this paper, we approach these problems from a Bayesian perspective covering general conjugate exponential models. Our proposal makes use of non-conjugate hierarchical priors to explicitly model temporal changes of the model parameters. We also derive a novel variational inference scheme which overcomes the use of non-conjugate priors while maintaining the computational efficiency of variational methods over conjugate models. The approach is validated on three real data sets over three latent variable models.

==> hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for å markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\boldsymbol{\Upsilon}$}}}
\nc{\bmupsilon}{{\mbox{\bm $\boldsymbol{\upsilon}$}}}
\nc{\bmalpha}{{\mbox{\bm $\boldsymbol{\alpha}$}}}
\nc{\bmbeta}{{\mbox{\bm $\boldsymbol{\beta}$}}}
\nc{\bmgamma}{{\mbox{\bm $\boldsymbol{\gamma}$}}}
\nc{\bmGamma}{{\mbox{\bm $$\boldsymbol{\Gamma}$}}}
\nc{\bmdelta}{{\mbox{\bm $\boldsymbol{\delta}$}}}
\nc{\bmDelta}{{\mbox{\bm $\boldsymbol{\Delta}$}}}
\nc{\bmeps}{{\mbox{\bm $\boldsymbol{\epsilon}$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\boldsymbol{\phi}$}}}
\nc{\bmPhi}{{\mbox{\bm $\$\boldsymbol{\Phi}$}}}
\nc{\bmlambda}{{\mbox{\bm $\boldsymbol{\lambda}$}}}
\nc{\bmLambda}{{\mbox{\bm $\boldsymbol{\Lambda}$}}}
\nc{\bmmu}{{\mbox{\bm $\boldsymbol{\mu}$}}}
\nc{\bmnu}{{\mbox{\bm $\boldsymbol{\nu}$}}}
\nc{\bmpi}{{\mbox{\bm $\boldsymbol{\pi}$}}}
\nc{\bmrho}{{\mbox{\bm$\boldsymbol{\rho}$}}}
\nc{\bmpsi}{{\mbox{\bm $\boldsymbol{\psi}$}}}
\nc{\bmPsi}{{\mbox{\bm $\boldsymbol{\Psi}$}}}
\nc{\bmsigma}{{\mbox{\bm $$\boldsymbol{\sigma}$}}}
\nc{\bmSigma}{{\mbox{\bm $\boldsymbol{\Sigma}$}}}
\nc{\bmtheta}{{\ensuremath{\boldsymbol{\theta}}}}
%\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
\nc{\bmeta}{{\ensuremath{\boldsymbol{\eta}}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


